Equivariant Littlewood-Richardson Skew Tableaux

We give a positive equivariant Littlewood-Richardson rule also discovered independently by Molev. Our proof generalizes a proof by Stembridge of the ordinary Littlewood-Richardson rule. We describe a weight-preserving bijection between our indexing tableaux and the Knutson-Tao puzzles.

==> apic13_tex.tex <==
\begin{center}

\psset{unit=2cm,linewidth=.15} \pspicture(0,-.5)(4.5,3)
%\psgrid[subgriddiv=1,griddots=10,gridlabels=10pt](0,0)(6,6)
%tableau
\psset{linewidth=.02}
%horizontal lines
\psline(3,3)(4,3) \psline(1,2)(4,2) \psline(0,1)(4,1)
\psline(0,0)(4,0)
%vertical lines
\psline(0,0)(0,1) \psline(1,0)(1,2) \psline(2,0)(2,2)
\psline(3,0)(3,3) \psline(4,0)(4,3)
%numbers
%bottom row
\rput{0}(1.5,.5){$y_6-y_5$}
%\rput{0}(4.5,2.5){$7,9$}
%2nd from bottom row
\rput{0}(2.5,1.5){$y_7-y_4$} \rput{0}(3.5,1.5){$y_4-y_1$}

%label the rows and columns
%rows
\rput{0}(4.2,.5){\tiny $4$}
\rput{0}(4.2,1.5){\tiny $3$}
\rput{0}(4.2,2.5){\tiny $2$}
%columns
\rput{0}(.5,-.2){\tiny $4$}
\rput{0}(1.5,-.2){\tiny $3$}
\rput{0}(2.5,-.2){\tiny $2$}
\rput{0}(3.5,-.2){\tiny $1$}

\endpspicture

\end{center}

